An Operational Guide to Monitorability

Monitorability delineates what properties can be verified at runtime. Although many monitorability definitions exist, few are defined explicitly in terms of the guarantees provided by monitors, i.e., the computational entities carrying out the verification. We view monitorability as a spectrum: the fewer monitor guarantees that are required, the more properties become monitorable. We present a monitorability hierarchy and provide operational and syntactic characterisations for its levels. Existing monitorability definitions are mapped into our hierarchy, providing a unified framework that makes the operational assumptions and guarantees of each definition explicit. This provides a rigorous foundation that can inform design choices and correctness claims for runtime verification tools.

==> monitorabilities.tex <==

%In the sequel we show that this operational hierarchy gives a concrete, uniform operational interpretation for various notions of monitorability that appear in the literature. The classical definitions that we will consider have a denotational flavour: they don't refer to monitors and to how monitor verdicts might relate to properties; rather, they consider directly the characteristics of a set of traces.

%%% moved to its section

\section{Safety and Co-safety}
\label{sec:safety}
\input{safety}


\section{Pnueli and Zaks}
\label{sec:pz}
\input{pz}

\section{Other related work}
\label{sec:other}
\input{ffm4}

